FPA-CS: Focal Plane Array-based Compressive Imaging in Short-wave Infrared

Cameras for imaging in short and mid-wave infrared spectra are significantly more expensive than their counterparts in visible imaging. As a result, high-resolution imaging in those spectrum remains beyond the reach of most consumers. Over the last decade, compressive sensing (CS) has emerged as a potential means to realize inexpensive short-wave infrared cameras. One approach for doing this is the single-pixel camera (SPC) where a single detector acquires coded measurements of a high-resolution image. A computational reconstruction algorithm is then used to recover the image from these coded measurements. Unfortunately, the measurement rate of a SPC is insufficient to enable imaging at high spatial and temporal resolutions. We present a focal plane array-based compressive sensing (FPA-CS) architecture that achieves high spatial and temporal resolutions. The idea is to use an array of SPCs that sense in parallel to increase the measurement rate, and consequently, the achievable spatio-temporal resolution of the camera. We develop a proof-of-concept prototype in the short-wave infrared using a sensor with 64$\times$ 64 pixels; the prototype provides a 4096$\times$ increase in the measurement rate compared to the SPC and achieves a megapixel resolution at video rate using CS techniques.

==> anal.tex <==
\subsection{PSF}
\subsection{Design of patterns}
 Random vs hadamard vs totally random
\subsection{MTF}
Frequency vs measurement rate \\
       Frequency vs snr
\subsection{Adapt to motion}
Plot of measurement rate vs psnr for different velocities\\
Use that data to create plot of primal measurement rate for particular velocity
\subsection{}

==> analysis.tex <==
We tested the performance of proposed system on simulated system matrix for noise and compression ratio analysis, and on actual system matrix from calibration for Modulation transfer function (MTF) analysis focused on the optical characteristics of our prototype system.

For the simulated system matrix A, we modeled it as 
\[
A = B_1 R M B_2,
\] 
where $B_2$ is the image degradation introduced by the  main objective lens, modeled as a Gaussian blur, $M$ is the spatial coding on the DMD, $R$ is the magnification introduced by the re-imaging lens that focuses the coded DMD image onto the sensor plane, modeled as a 8x down-sampling process, and $B_1$ is the degradation introduced by the re-imaging lens, again, modeled as a Gaussian blur. We input a vectorized natural image x, and simulated the measurements y = Ax using the constructed system matrix A. We then used sparse reconstruction algorithm to solve for $ \hat{x} $, and compared the results with the input image.

For the actual system matrix, we captured the matrix through our calibration process, in which we exhaustively measured the response of each DMD element on the SWIR area sensor. Given the response function is actually local, we perform the calibration in a parallel fashion: we divided the entire DMD plane and the corresponding SWIR area into 18x20 neighbourhood, and take measurements for those 360 neighbourhood simultaneously, and repeat it for the rest of elements in the neighbourhood. This parallel process significantly accelerated the calibration.

Using the acquired system matrix, we simulated the response $y$ of given input image $x$. We then solved for the reconstructed image $ \hat{x}$.


\vspace{-2mm}
\paragraph{Noise and Compression Ratio Analysis.}

To analyse the effect of compression ratio to the reconstruction performance, we run reconstruction experiments on with different amount of measurements taken. We also add different amount of measurement noise to see the noise's contribution to the reconstruction degradation. Specifically, we set the number of measurement to correspond 100.00\%, 50.00\%, 25.00\$, 12.50\%, 6.25\%, 3.13\% and 1.56\% compression ratio, and noise to be additive white Gaussian noise with signal-to-noise ratio of 10 dB, 20 dB, 30 dB and 40 dB. The reconstruction results are shown in Figure \ref{fig:analysis}. We also plot out the reconstruction results using peak signal-to-noise ratio (PSNR) and structural similarity (SSIM) as quality assessment metrics in each of those cases, compared to the original input image, in Figure \ref{fig:PSNR} and \ref{fig:SSIM} 

\begin{figure}[t]
	%\includegraphics[width=0.6\textwidth]{Figures/PSNR.eps}
	\includegraphics[width=0.475\textwidth, keepaspectratio]{Figures/PSNR.eps}	
	\caption{PSNR of the reconstruction results compared to the original input image at different compression ratio and with different amount of measurement noise added}
	\label{fig:PSNR}
\end{figure}

\begin{figure}[t]
	%\includegraphics[width=0.6\textwidth]{Figures/PSNR.eps}
	\includegraphics[width=0.475\textwidth, keepaspectratio]{Figures/SSIM.eps}	
	\caption{SSIM of the reconstruction results compared to the original input image at different compression ratio and with different amount of measurement noise added.}
	\label{fig:SSIM}
\end{figure}

\begin{figure*}[t]
	\centering
	\includegraphics[trim = 0mm 30mm 0mm 30mm, clip=true, width=1\textwidth, keepaspectratio]{Figures/Analysis}
	\caption{Reconstruction results at different compression ratio and measurement noise applied}
	\label{fig:analysis}
\end{figure*}

As expected, as noise level and compression ratio increases, the overall reconstruction quality decreases.
One important fact to note is that while devices such as the SPC can typically achieve a higher compression rate, FPA-CS only achieves smaller compression rates.
This is because, the global nature of the multiplexing in the SPC allows for greater reductions in measurements compared to the block-diagonal structure of the multiplexing matrix in FPA-CS.
Although the raw compression rate for FPA-CS is slightly lower, the three order of magnitude improvement in measurement rate achieved due to $4096$ parallel measurements, compensates for the small reduction in compression rate.
This is because both FPA-CS and SPC require synchronization between DMD and sensor and this is restricted to be at a rate no greater than $F_{max}$.
As a consequence, the practical temporal resolution that can be achieved by FPA-CS far exceeds that of an SPC.
In particular, SPC can only match the temporal resolution of FPA-CS if it can achieve a compression rate of $4000$, which is impractical.
Existing SPC systems typically achieve only compression rates of the order of $\alpha \approx 10-20$, resulting in FPA-CS achieving a temporal resolution that is at-least an order of magnitude better.

\vspace{-2mm}
\paragraph{MTF Analysis}
We study the spatial frequency response of our prototype FPA-CS system via its MTF.
Figure \ref{fig:MTF} shows the MTF of our system at varying compression rates.
First, note the dramatic improvement in MTF of multiplexed reconstruction (i.e., $\alpha=0.5,1,2,4$) compared to the raw sensor MTF (i.e., $\alpha=256$).
Secondly, note the gradual improvement in MTF with additional measurements, allowing the possibility for adaptive systems where the number of measurements used is adaptively chosen based on the estimated motion.
\begin{figure}[t]
	\includegraphics[width=0.5\textwidth]{Figures/MTF-New.eps}
	% \includegraphics[width=0.475\textwidth, keepaspectratio]{Figures/MTF_FPACS}	
	\caption{Modulation Transfer Function: The MTF of all imaging system at various compression rates $\alpha$ demonstrates the gradual degradation of higher spatial frequencies as the compression rate is increased.}
	\label{fig:MTF}
\end{figure}


\paragraph{Artifacts}

When reconstructing videos frame-by-frame without spatio-temporal prior, artifacts can be observed. We expect the artifacts to come from 

Using a 3D median filter, the artifacts can be reduced. The results with 3D median filter are shown in Figure \ref{fig:2hands_median}.

==> definitions.tex <==
\newcommand{\sinc}{\mathrm{sinc}}
\newcommand{\mA}{\ensuremath{\mathbf A}}
\newcommand{\mB}{\ensuremath{\mathbf B}}
\newcommand{\mC}{\ensuremath{\mathbf C}}
\newcommand{\mD}{\ensuremath{\mathbf D}}
\newcommand{\mF}{\ensuremath{\mathbf F}}
\newcommand{\mP}{\ensuremath{\mathbf P}}
\newcommand{\mQ}{\ensuremath{\mathbf Q}}
\newcommand{\mI}{\ensuremath{\mathbf I}}
\newcommand{\mU}{\ensuremath{\mathbf U}}
\newcommand{\mW}{\ensuremath{\mathbf W}}

\newcommand{\cA}{\ensuremath{\mathcal A}}
\newcommand{\cF}{\ensuremath{\mathcal F}}
\newcommand{\cM}{\ensuremath{\mathcal M}}
\newcommand{\cP}{\ensuremath{\mathcal P}}

\newcommand{\va}{\ensuremath{\mathbf a}}
\newcommand{\vb}{\ensuremath{\mathbf b}}
\newcommand{\vd}{\ensuremath{\mathbf d}}
\newcommand{\ve}{\ensuremath{\mathbf e}}
\newcommand{\vf}{\ensuremath{\mathbf f}}
\newcommand{\vg}{\ensuremath{\mathbf g}}
\newcommand{\vh}{\ensuremath{\mathbf h}}
\newcommand{\vn}{\ensuremath{\mathbf n}}
\newcommand{\vp}{\ensuremath{\mathbf p}}
\newcommand{\vq}{\ensuremath{\mathbf q}}
\newcommand{\vr}{\ensuremath{\mathbf r}}
% \newcommand{\vs}{\ensuremath{\mathbf s}}
\newcommand{\vu}{\ensuremath{\mathbf u}}
\newcommand{\vv}{\ensuremath{\mathbf v}}
\newcommand{\vw}{\ensuremath{\mathbf w}}
\newcommand{\vx}{\ensuremath{\mathbf x}}
\newcommand{\vy}{\ensuremath{\mathbf y}}
\newcommand{\vz}{\ensuremath{\mathbf z}}
\newcommand{\vpsi}{\ensuremath{\mathbf \psi}}
\newcommand{\vphi}{\ensuremath{\mathbf \phi}}
\newcommand{\mPsi}{\ensuremath{\mathbf \Psi}}
\newcommand{\mPhi}{\ensuremath{\mathbf \Phi}}
\newcommand{\ct}{\ensuremath{\widetilde{c}}}
\newcommand{\setT}{\ensuremath{\mathcal T}}
\newcommand{\proj}{\ensuremath{\mathcal P}}
\newcommand{\rf}[1]{\ensuremath{{\mathbf \phi}_{#1}}}
\newcommand{\af}[1]{\ensuremath{\underline{\mathbf f}_{#1}}}
\newcommand{\ru}[1]{\ensuremath{{\mathbf u}_{#1}}}
\newcommand{\qa}[1]{\ensuremath{\hat{a}_{#1}}}
\newcommand{\comp}[2]{\ensuremath{c_{#1,#2}}}
\newcommand{\resid}[2]{\ensuremath{\vr_{#1,#2}}}
\newcommand{\cerr}[2]{\ensuremath{\ct_{#1,#2}}}
\newcommand{\vsW}{\ensuremath{\mathcal{W}}}
\newcommand{\vsS}{\ensuremath{\mathcal{S}}}
\newcommand{\vsH}{\ensuremath{\mathcal{H}}}
\newcommand{\opF}{\ensuremath{\mathbf{F}}}
\newcommand{\piF}{\ensuremath{\mathbf{F}^\dagger}}
\newcommand{\adjF}{\ensuremath{\mathbf{F}^*}}
\newcommand{\Epsilon}{\ensuremath{\mathcal{E}}}
\newcommand{\Reals}{\ensuremath{\mathbb{R}}}
\newcommand{\SD}{\ensuremath{\Sigma\Delta}}
\newcommand{\deq}{\ensuremath{ \overset{\text{def}}{=} }}
\newcommand{\MMSE}{\ensuremath{\mbox{MMSE}}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator{\sign}{sign}
%\DeclareMathOperator{\diag}{diag}
\newcommand{\supp}[1]{\ensuremath{\operatorname{supp}\left(#1\right)}}
\newcommand{\diag}[1]{\ensuremath{\operatorname{diag}\left(#1\right)}}
\newcommand{\nullsp}[1]{\ensuremath{\operatorname{null}(#1)}}
\newcommand{\range}[1]{\ensuremath{\operatorname{range}(#1)}}
\renewcommand{\dim}[1]{\ensuremath{\operatorname{dim}(#1)}}
\newcommand{\spanof}[1]{\ensuremath{\operatorname{span}\{#1\}}}
\newcommand{\rankof}[1]{\ensuremath{\operatorname{rank}\{#1\}}}

%--------------------------------------------------------------------------

% Homotopy
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\R}{\mathbb{R}}
\newcommand{\sgn}{\operatorname{sgn}}
\renewcommand{\P}{\operatorname{P}}
\newcommand{\E}{\operatorname{E}}
\newcommand{\deps}{\Delta \epsilon}
\newcommand{\delx}{\ensuremath{\partial \mathbf{x}}}

\newcommand{\field}[1]{\mathbb{#1}}                                   % Topological sets
\newcommand{\prn}[1]{\left(#1\right)}                                 % Parenthetical
\newcommand{\Prn}[1]{\left[#1\right]}                                 % Parenthetical 2
\newcommand{\clog}[1]{\textnormal{Log}\left(#1\right)}                % Complex Logarithm
\newcommand{\cfn}[2]{#1\left(#2\right)}                               % Continuous function
\newcommand{\dfn}[2]{#1\left[#2\right]}                               % Discrete function
\newcommand{\dff}[2]{\displaystyle\frac{d#1}{d#2}}                    % Differential (fraction form)
\newcommand{\dfe}[2]{\displaystyle\frac{d}{d#2}\left(#1\right)}       % Differential (expression form)
\newcommand{\pdff}[2]{\displaystyle\frac{\partial #1}{\partial #2}}   % Partial Differential (fraction form)
\newcommand{\pdfe}[2]{\displaystyle\frac{\partial}{\partial #2}#1}    % Partial Differential (expression form)
\newcommand{\pdo}[1]{\displaystyle\frac{\partial}{\partial #1}}       % Partial Differential Operator
% dfrac:   \newcommand{\nfrac}[2]{\displaystyle\frac{#1}{#2}}                    % Display Fraction
\newcommand{\dlim}[2]{\displaystyle\lim_{#1}\left(#2\right)}          % Display Limit
\newcommand{\dint}[3]{\displaystyle\int_{#1}^{#2}{#3}}                % Display Integral
\newcommand{\dsum}[3]{\displaystyle\sum_{#1}^{#2}{#3}}                % Display Sum
\newcommand{\centerup}[1]{\begin{center}#1\end{center}}               % Center text
\newcommand{\HRule}{\rule{\linewidth}{0.5mm}}                         % Horizontal line
\newcommand{\abs}[1]{\left|#1\right|}                                 % Absolute value
\newcommand{\elone}[1]{\left\|#1\right\|_1}                           % L-1 Norm
\newcommand{\eltwo}[1]{\left\|#1\right\|_2}                           % L-2 Norm
\newcommand{\elinf}[1]{\left\|#1\right\|_\infty}                      % L-infinity Norm
\newcommand{\fro}[1]{\left\|#1\right\|_{fro}}                         % Frobenius Norm
\newcommand{\norm}[1]{\left\|#1\right\|}                              % Norm
\renewcommand{\labelenumi}{(\alph{enumi})}                            % To get enumerate to display letters
\newcommand{\ip}[1]{\langle{#1}\rangle}																 % Inner Product
\newcommand{\sarray}[1]{\begin{array}{l}#1\end{array}}								 % simple array
\newcommand{\sarrayc}[1]{\begin{array}{c}#1\end{array}}								 % simple array (center)
\newcommand{\darray}[1]{\begin{array}{ll}#1\end{array}}								 % double array
\newcommand{\darraycl}[1]{\begin{array}{cl}#1\end{array}}							 % double array (center,left)
\newcommand{\res}[1]{\centerup{\framebox{#1}}}												 % Important result (centered and boxed)
\newcommand{\amatrix}[1]{\begin{bmatrix}#1\end{bmatrix}}							 % matrix (bmatrix)
\newcommand{\minim}[2]{\underset{#1}{\min}{#2}}												 % minimize
\newcommand{\maxim}[2]{\underset{#1}{\max}{#2}}												 % maximize
\newcommand{\sign}[1]{\mathrm{sign}{\left(#1\right)}}									 % sign function
%
% Theorems, Lemmas, Proposition...
%
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{definition}{Definition}[section]

% \newcommand{\qed}{\framebox{}}
%\newtheorem{thm}{Theorem}[chapter]
%\theoremstyle{definition}
%\newtheorem{dfn}{Definition}[chapter]
%\theoremstyle{remark}
%\newtheorem{note}{Note}[chapter]
%\theoremstyle{plain}
%\newtheorem{lem}[thm]{Lemma}
%\newtheorem{corr}[thm]{Corrollary}
%\newtheorem{prop}[thm]{Proposition}
%
% LCA Symbols
%
\newcommand{\G}{\Gamma}
\newcommand{\Gc}{\Gamma^c}
\newcommand{\g}{\gamma}
\newcommand{\PP}{\Phi_{\Gamma}^T\Phi_{\Gamma}}
\newcommand{\PcP}{\Phi_{\Gamma^c}^T\Phi_{\Gamma}}
%
% Custom Trig functions
%
\newcommand{\cosine}[1]{\mathbf{\cos}\left(#1\right)}
\newcommand{\sine}[1]{\mathbf{\sin}\left(#1\right)}
\newcommand{\cosinep}[2]{\mathbf{\cos}^{#2}\left(#1\right)}
\newcommand{\sinep}[2]{\mathbf{\sin}^{#2}\left(#1\right)}
\newcommand{\tangent}[1]{\tan\left(#1\right)}
\newcommand{\cosecant}[1]{\csc\left(#1\right)}
\newcommand{\secant}[1]{\sec\left(#1\right)}
\newcommand{\cotangent}[1]{\cot\left(#1\right)}
\newcommand{\arctangent}[1]{\tan^{-1}\left(#1\right)}
\newcommand{\arcsine}[1]{\arcsin\left(#1\right)}
\newcommand{\arccosine}[1]{\arccos\left(#1\right)}
\newcommand{\hypsine}[1]{\sinh\left(#1\right)}
\newcommand{\hypcosine}[1]{\cosh\left(#1\right)}
\newcommand{\hyptangent}[1]{\tanh\left(#1\right)}
\newcommand{\atanq}[2]{\arctangent{\gfrac{#1}{#2}}}
%
% Custom tabbing
%
\newcommand{\etab}{\ \ \ \ }
\newcommand{\dnl}{\newline\newline}                                  % Double newline
%
% Probability Functions
%
\newcommand{\expc}[1]{E\left[#1\right]}	                             % Expectation
\newcommand{\expco}[2]{E\left[\left.#1\right|#2\right]}              % Conditional Expectation
\newcommand{\exps}[2]{E_{#1}\left[#2\right]}                         % Expectation with subscript
\newcommand{\var}[1]{\texttt{var}\func{#1}}		                       % Variance
\newcommand{\vars}[2]{\texttt{var}_{#1}\func{#2}}                    % Variance with subscript
\newcommand{\cov}[1]{\texttt{cov}\func{#1}}		                       % Covariance
\newcommand{\pdf}[2]{\mkfunc{f_{#1}}{#2}}                            % Probability Distribution Function
\newcommand{\pr}[1]{Pr\func{#1}} 						                         % Probability
%
% Probability Distributions
%
\newcommand{\gaussian}[1]{\dfrac{1}{\sqrt{2\pi\sigma_{#1}^2}}e^{-\frac{\prn{#1-\mu_{#1}}^2}{2\sigma_{#1}^2}}}
%
% Figure
%
%\newcommand{\fig}[4]{\begin{figure}
%\begin{center}
%\includegraphics[width=#1]{#2}
%\caption{#3}
%\label{fig:#4}
%\end{center}
%\end{figure}}
%%
%\newcommand{\figh}[4]{\begin{figure}[h]
%\begin{center}
%\includegraphics[width=#1]{#2}
%\caption{#3}
%\label{fig:#4}
%\end{center}
%\end{figure}}


%
%--------------------------------------------------------------------------


\newcommand{\PBnote}[1]{{\em [**PB:{#1}]}}
\newcommand{\Salnote}[1]{{\color{red}[{\em SA:{#1} ??}]}}
\newcommand{\TBC}[1][]{\todo[inline]{To be continued...?? \\ {#1}}}


%--------------------------------------------------------------------------
% Revise/annotate
\newif\ifannotated

\annotatedfalse

\ifannotated
% draft
\newcommand{\add}[1]{{\color{blue}{#1}}}
\newcommand{\delete}[1]{{\color{red}{\sout{#1}}}}
\newcommand{\replace}[2]{{\delete{#1}} -:- {\add{#2}}}
\newcommand{\margincomment}[1]{\marginpar{$\Rightarrow$\color{red}\fbox{\parbox{\linewidth}{\color{black}\scriptsize#1}}}}
\else
% final
\newcommand{\add}[1]{{{#1}}}
\newcommand{\delete}[1]{{\unskip \ignorespaces}}
\newcommand{\replace}[2]{{\add{#2}}}
\newcommand{\margincomment}[1]{}
\fi

% \newcommand{\replace}[2]{{\color{red}{\underline{#1}}}{\color{blue}{\sout{#2}}}}
% \newcommand{\add}[1]{{\color{red}{\underline{#1}}}}
% \newcommand{\delete}[1]{{\color{red}{\sout{#1}}}}
% \newcommand{\margincomment}[1]{\marginpar{$\Rightarrow$\color{red}\fbox{\parbox{\linewidth}{\color{black}\scriptsize#1}}}}
%
%ex )  axial slices \margincomment{In response to R1.2, texts are
%revised}\replace{(thickness = 3 mm; gap = 0.6 mm)}{with 20\% gap,
%thickness = 3 mm}, TE = 30 msec
%-------------------------------------------------------------------------------

%
%\newcommand*\Let[2]{\State #1 $\gets$ #2}
%%\algrenewcommand\alglinenumber[1]{{\sf\footnotesize\addfontfeatures{Color=888888,Numbers=Monospaced}#1}}
%\algrenewcommand\algorithmicrequire{\textbf{Input:}}
%\algrenewcommand\algorithmicensure{\textbf{Output:}}
%\algrenewcommand\algorithmicrepeat{\textbf{Repeat:}}

%--------------------------------------------------------------------------



%% Abstract
%Motivation:
%Why do we care about the problem and the results? If the problem isn't obviously "interesting" it might be better to put motivation first; but if your work is incremental progress on a problem that is widely recognized as important, then it is probably better to put the problem statement first to indicate which piece of the larger problem you are breaking off to work on. This section should include the importance of your work, the difficulty of the area, and the impact it might have if successful.
%Problem statement:
%What problem are you trying to solve? What is the scope of your work (a generalized approach, or for a specific situation)? Be careful not to use too much jargon. In some cases it is appropriate to put the problem statement before the motivation, but usually this only works if most readers already understand why the problem is important.
%Approach:
%How did you go about solving or making progress on the problem? Did you use simulation, analytic models, prototype construction, or analysis of field data for an actual product? What was the extent of your work (did you look at one application program or a hundred programs in twenty different programming languages?) What important variables did you control, ignore, or measure?
%Results:
%What's the answer? Specifically, most good computer architecture papers conclude that something is so many percent faster, cheaper, smaller, or otherwise better than something else. Put the result there, in numbers. Avoid vague, hand-waving results such as "very", "small", or "significant." If you must be vague, you are only given license to do so when you can talk about orders-of-magnitude improvement. There is a tension here in that you should not provide numbers that can be easily misinterpreted, but on the other hand you don't have room for all the caveats.
%Conclusions:
%What are the implications of your answer? Is it going to change the world (unlikely), be a significant "win", be a nice hack, or simply serve as a road sign indicating that this path is a waste of time (all of the previous results are useful). Are your results general, potentially generalizable, or specific to a particular case?
% Motivation
% Problem statement
% Approach
% Results
% Conclusions

% References: 
% http://klab.smpp.northwestern.edu/wiki/index.php5/Paper_Writing_101
% 

==> mode.tex <==
Our prototype is a flexible imaging framework that can be utilized for different novel computational imaging tasks in addition to compressive sensing, here  we show a few samples.


\vspace{-2mm}
\paragraph{Optical super-resolution (SR)}
The idea of super resolution implemented in optics domain was first presented in \cite{ben2004jitter}, in which the technique is termed ``Jitter Camera''. 

To super-resolve an image $I(x,y), {x,y} \in \mathbb{N}$, one wish to  resolve the intensity value at subpixel locations:
\[
I(x+u, y+v), (x,y) \in \mathbb{N}, (u,v) \in (0,1)
\]
In \cite{ben2004jitter}, the author implemented a floating sensor plane that can be moved with sub-pixel distance using a actuator %(Figure \ref{fig:jitter})
, which enabled them to perform sub-pixel sampling.


On FPA-CS, optical super-resolution can be achieved without the precise actuator.  In our proposed architecture, each pixel (i.e. macro-pixel) on the sensor is mapped to an area consisted of 16x16 pixels (i.e. micro-pixel) on the DMD. Since the micro-pixels are spatiotemporally programmable and synchronized with the macro-pixel, we are able to modulate the light throughput on each of the micro-pixels, and sample at macro-pixel. For instance, given a scene $I$, sub-pixel measurements 
\[
I(x + u/16, y+v/16), (x,y) \in [0, 64], 
\]
\[
(x,y) \in \mathbb{N}, (u,v) \in (0, 16), (u,v) \in \mathbb{R}
\]
can be taken from macro-pixels $I(x,y), (x,y) \in [0, 64],  (x,y) \in  \mathbb{N}$, if we take 256 marco-pixel sensor measurements, with a different micro-pixel in the 16x16 neighborhood turned on each time, we are able to take 256 non-overlapping sub-pixel measurements at each given macro-pixel.  As a result, we can easily achieve optical super-resolution at 16x, which can hardly be reached using conventional super-resolution technique. We show the optical SR results on the side of state-of-the-art SR algorithm \cite{babacan2011variational} in Figure \ref{fig:SR}.

\begin{figure}[t]
	%\includegraphics[width=0.5\textwidth]{Figures/SR.pdf}
	\includegraphics[width=0.475\textwidth, keepaspectratio]{Figures/SR}	
	\caption{Original 64x64 image (a), 2x SR of the original image using state-of-the-art SR algorithm \cite{babacan2011variational} (b), and ~16x optical SR of the original image using FPA-CS}
	\label{fig:SR}
\end{figure}

